Understanding Model Selection For Learning In Strategic Environments

The deployment of ever-larger machine learning models reflects a growing consensus that the more expressive the model class one optimizes over$\unicode{x2013}$and the more data one has access to$\unicode{x2013}$the more one can improve performance. As models get deployed in a variety of real-world scenarios, they inevitably face strategic environments. In this work, we consider the natural question of how the interplay of models and strategic interactions affects the relationship between performance at equilibrium and the expressivity of model classes. We find that strategic interactions can break the conventional view$\unicode{x2013}$meaning that performance does not necessarily monotonically improve as model classes get larger or more expressive (even with infinite data). We show the implications of this result in several contexts including strategic regression, strategic classification, and multi-agent reinforcement learning. In particular, we show that each of these settings admits a Braess' paradox-like phenomenon in which optimizing over less expressive model classes allows one to achieve strictly better equilibrium outcomes. Motivated by these examples, we then propose a new paradigm for model selection in games wherein an agent seeks to choose amongst different model classes to use as their action set in a game.

==> newcommands.tex <==
%%%%%% ENVIRONMENTS %%%%%%
%\swapnumbers
%\newtheorem{theorem}{Theorem}
%\newtheorem{proposition}[theorem]{Proposition}
%\newtheorem{lemma}[theorem]{Lemma}
%\newtheorem{definition}[theorem]{Definition}
%\newtheorem{corollary}[theorem]{Corollary}
%\newtheorem{remark}[theorem]{Remark}
%\newtheorem{conjecture}[theorem]{Conjecture}
%\newtheorem{notation}[theorem]{Notation}
%\newtheorem{example}[theorem]{Example}
%\newtheorem{exercise}{Exercise}
%\newtheorem*{notes}{Notes}


%\newtheorem{theorem}{Theorem}[section]
%\newtheorem{lemma}[theorem]{Lemma}
\newtheorem{corollary}{Corollary}
\newtheorem{proposition}[theorem]{Proposition}
%\newtheorem{definition}[theorem]{Definition}
%\newtheorem{claim}{Claim}
\newtheorem{conjecture}[theorem]{Conjecture}
\newtheorem{observation}[theorem]{Observation}
\newtheorem{problem}[theorem]{Problem}
\newtheorem{example}[theorem]{Example}
\newtheorem*{theorem*}{Theorem}
\newtheorem*{example*}{Example}
\newtheorem*{corollary*}{Corollary}



%%%%%% NEW COMMANDS/OPERATORS %%%%%%
\DeclareMathOperator{\esup}{\text{ess\;sup}}
\providecommand{\abs}[1]{\lvert#1\rvert} % absolute value function
\renewcommand{\P}{\mathbb{P}}  % probability measure
\renewcommand{\O}{\mathcal{O}} % order notation
\newcommand{\PP}{\P^\star} % pricing probability measure
\newcommand{\E}{\mathbb{E}}  % expectation
\newcommand{\Var}{\mathrm{Var}}
\newcommand{\EE}{\E^\star}   % expectation under the pricing measure
\newcommand{\V}{\text{Var}} % variance
\newcommand{\F}{\mathcal{F}} % filtration
\newcommand{\G}{\mathcal{G}} % filtration
\renewcommand{\H}{\mathcal{H}} % filtration
\newcommand{\Fb}{\mathbb{F}} % filtration
\newcommand{\N}{\mathbb{N}}  % integers
\newcommand{\R}{\mathbb{R}}  % real numbers
%\renewcommand{\C}{\mathbb{C}}  % complex numbers
\newcommand{\argmin}{\mathop{\mathrm{arg\,min}}} % arg min operator
\newcommand{\argmax}{\mathop{\mathrm{arg\,max}}}
\newcommand{\cpb}{c^{\mbox{\scriptsize pb}}} % protection buyer payment
\newcommand{\cps}{c^{\mbox{\scriptsize ps}}} % protection seller payment
\newcommand{\cds}{c^{\mbox{\scriptsize ds}}} % CDS spread

\newcommand{\T}{\mathcal{T}} % tenor
\renewcommand{\vec}[1]{\mbox{\boldmath $#1$}} % boldface 1 for the indicator function
\newcommand{\ind}{\vec{1}}                    % boldface 1 for the indicator function
\newcommand{\Ws}{W^\star_t}
\newcommand{\tWs}{\widetilde{W}^\star_t}
\newcommand{\tWz}{\widetilde{W}^0_t}
\newcommand{\tW}{\widetilde{W}}

%%%%%% Shortcut expressions %%%%%%
\newcommand{\pb}{protection buyer}
\newcommand{\ps}{protection seller}
\newcommand{\BibTeX}{{\sc Bib}\TeX}

%%%%%% Greeks %%%%%%
\newcommand{\eps}{\varepsilon}
\newcommand{\de}{\delta}
\newcommand{\fee}{\varphi}
\newcommand{\half}{\frac{1}{2}}

%%%%%% PDEs %%%%%%%
\newcommand{\pa}{\partial}
\renewcommand{\L}{\mathcal{L}}
\newcommand{\M}{\mathcal{M}}
\newcommand{\A}{\mathcal{A}}
\newcommand{\wA}{\widetilde{\A}}
\newcommand{\wlop}{\widetilde{\L}}
\newcommand{\wmop}{\widetilde{\M}}
\newcommand{\lbs}{\L_{BS}}
\newcommand{\lbss}{\L_{BS^\star}}
\newcommand{\lzero}{\L_{0}}
\newcommand{\lone}{\L_{1}}
\newcommand{\ltwo}{\L_{2}}
\newcommand{\wled}{\widetilde{\L}^{\eps,\de}}
\newcommand{\wlone}{\widetilde{\L}_1}
\newcommand{\wltwo}{\widetilde{\L}_2}
\newcommand{\cltwo}{\langle \L_2 \rangle}
\newcommand{\cwltwo}{\left\langle \wltwo \right\rangle}
\newcommand{\mone}{\M_{1}}
\newcommand{\mtwo}{\M_{2}}
\newcommand{\mthree}{\M_{3}}
\newcommand{\wmone}{\widetilde{\M}_1}
\newcommand{\fc}{\langle f \rangle}  % <f>

\newcommand{\bes}{\begin{equation*}}

%%%%%% OLD ONES %%%%%%
%\newcommand{\sigbar}{\overline{\sigma}}
%\newcommand{\sigstar}{\sigma_\star}
%\newcommand{\CBS}{C_{BS}}
%\newcommand{\CBSs}{C_{BS^\star}}
%\newcommand{\BS}{Black-Scholes }
%\newcommand{\vol}{volatility}
%\newcommand{\SV}{stochastic volatility }
%\newcommand{\PP}{{\mathord{I\kern -.33em P}}}
%\newcommand{\EE}{{\mathord{I\kern -.33em E}}}
%\newcommand{\RR}{{\mathord{I\kern -.33em R}}}
%\newcommand{\1}{{\mathord{1\kern -.26em \text{I}}}}
%\newcommand{\calp}{{\PP}}
%\newcommand{\EEE}{{\EE^{\star}}}
%\newcommand{\PPP}{{\PP^{\star}}}
%\newcommand{\ssb}{\overline{\sigma^2}}

